A Factorization Approach to Inertial Affine Structure from Motion

We consider the problem of reconstructing a 3-D scene from a moving camera with high frame rate using the affine projection model. This problem is traditionally known as Affine Structure from Motion (Affine SfM), and can be solved using an elegant low-rank factorization formulation. In this paper, we assume that an accelerometer and gyro are rigidly mounted with the camera, so that synchronized linear acceleration and angular velocity measurements are available together with the image measurements. We extend the standard Affine SfM algorithm to integrate these measurements through the use of image derivatives.

==> figures/sketch/imu_quadrotor_image.tex <==
% Sketch output, version 0.3 (build 7d, Sat Sep 26 10:35:44 2015)
% Output language: PGF/TikZ,LaTeX

\filldraw[fill=white](-5.605,1.967)--(-6.027,2.077)--(-6.027,.439)--(-5.182,-.601)--(-5.182,1.038)--cycle;
\filldraw[fill=white](-3.792,2.452)--(-4.215,2.562)--(-6.027,2.077)--(-5.605,1.967)--cycle;
\draw[color=gray](2.703,-.569)--(2.698,-.568);
\filldraw[fill=gray,draw=none](2.539,-.446)--(2.779,-.771)--(2.788,-.686)--(2.547,-.361)--cycle;
\draw(2.539,-.446)--(2.779,-.771);
\draw(2.788,-.686)--(2.547,-.361);
\draw[color=gray](2.335,-.506)--(.401,-.178);
\draw(.137,.645)--(-3.792,2.452);
\filldraw[fill=Azure2,fill opacity=0.5](-.379,.602)--(-.625,-1.795)--(.401,-.178)--(.647,2.219)--cycle;
\filldraw[fill=white](-3.37,-.116)--(-3.37,1.523)--(-5.182,1.038)--(-5.182,-.601)--cycle;
\filldraw[fill=brown](-4.272,-.363)--(-3.818,-.242)--(-3.818,.577)--(-4.272,.456)--cycle;
\filldraw[fill=white](-3.37,1.523)--(-3.792,2.452)--(-5.605,1.967)--(-5.182,1.038)--cycle;
\draw(.268,.585)--(.137,.645);
\filldraw[fill=white](.177,.321)--(.105,-.413)--(.27,-.049)--(.326,.549)--(.273,.606)--cycle;
\filldraw[fill=white](.105,-.413)--(.177,.321)--(-.035,-.019)--(-.098,-.63)--cycle;
\filldraw[fill=brown](-.007,-.534)--(.045,-.478)--(.081,-.123)--(.027,-.196)--cycle;
\filldraw[fill=gray,draw=none](2.399,-.256)--(2.539,-.446)--(2.547,-.361)--(2.408,-.172)--cycle;
\draw(2.547,-.361)--(2.408,-.172)--(2.399,-.256)--(2.539,-.446);
\draw[arrows=-,line width=2pt,color=Maroon1](2.819,-.648)--(2.819,-1.293);
\filldraw[fill=gray,draw=none](2.408,-.172)--(2.788,-.686)--(2.883,-.666)--(2.504,-.151)--cycle;
\draw(2.883,-.666)--(2.504,-.151)--(2.408,-.172)--(2.788,-.686);
\filldraw[fill=gray,fill opacity=0.5,draw=none](2.746,-.109)--(2.772,-.165)--(2.768,-.221)--(2.736,-.271)--(2.678,-.312)--(2.601,-.338)--(2.511,-.347)--(2.417,-.339)--(2.37,-.326)--(2.196,-.09)--(2.213,-.063)--(2.271,-.022)--(2.349,.004)--(2.439,.013)--(2.532,.005)--(2.62,-.02)--(2.694,-.059)--cycle;
\draw[draw=gray!50!black,draw opacity=0.5](2.196,-.09)--(2.213,-.063)--(2.271,-.022)--(2.349,.004)--(2.439,.013)--(2.532,.005)--(2.62,-.02)--(2.694,-.059)--(2.746,-.109)--(2.772,-.165)--(2.768,-.221)--(2.736,-.271)--(2.678,-.312)--(2.601,-.338)--(2.511,-.347)--(2.417,-.339)--(2.37,-.326);
\draw[color=gray](2.019,.445)--(.647,2.219);
\draw[arrows=-latex,line width=2pt,color=Maroon1](2.819,-1.293)--(2.819,-1.817);
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.439,.013)--(2.451,.133)--(2.544,.125)--(2.532,.005)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.532,.005)--(2.544,.125)--(2.632,.1)--(2.62,-.02)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.349,.004)--(2.361,.124)--(2.451,.133)--(2.439,.013)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.62,-.02)--(2.632,.1)--(2.706,.061)--(2.694,-.059)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.271,-.022)--(2.283,.098)--(2.361,.124)--(2.349,.004)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.694,-.059)--(2.706,.061)--(2.758,.011)--(2.746,-.109)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.213,-.063)--(2.226,.057)--(2.283,.098)--(2.271,-.022)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.746,-.109)--(2.758,.011)--(2.784,-.045)--(2.772,-.165)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.181,-.113)--(2.194,.007)--(2.226,.057)--(2.213,-.063)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.772,-.165)--(2.784,-.045)--(2.78,-.101)--(2.768,-.221)--cycle;
\filldraw[fill=gray](2.415,-.167)--(2.428,-.048)--(2.428,-.036)--(2.416,-.156)--cycle;
\filldraw[fill=gray](2.533,-.178)--(2.546,-.058)--(2.539,-.068)--(2.527,-.188)--cycle;
\filldraw[fill=gray](2.42,-.178)--(2.433,-.059)--(2.428,-.048)--(2.415,-.167)--cycle;
\filldraw[fill=gray](2.527,-.188)--(2.539,-.068)--(2.528,-.076)--(2.515,-.196)--cycle;
\filldraw[fill=gray](2.431,-.188)--(2.443,-.069)--(2.433,-.059)--(2.42,-.178)--cycle;
\filldraw[fill=gray](2.515,-.196)--(2.528,-.076)--(2.512,-.081)--(2.5,-.201)--cycle;
\filldraw[fill=gray](2.446,-.196)--(2.458,-.077)--(2.443,-.069)--(2.431,-.188)--cycle;
\filldraw[fill=gray](2.5,-.201)--(2.512,-.081)--(2.494,-.083)--(2.482,-.203)--cycle;
\filldraw[fill=gray](2.463,-.201)--(2.476,-.082)--(2.458,-.077)--(2.446,-.196)--cycle;
\filldraw[fill=gray](2.482,-.203)--(2.494,-.083)--(2.476,-.082)--(2.463,-.201)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.706,.061)--(2.632,.1)--(2.544,.125)--(2.451,.133)--(2.361,.124)--(2.283,.098)--(2.226,.057)--(2.194,.007)--(2.19,-.049)--(2.216,-.105)--(2.268,-.155)--(2.342,-.194)--(2.43,-.219)--(2.523,-.228)--(2.613,-.218)--(2.691,-.192)--(2.748,-.151)--(2.78,-.101)--(2.784,-.045)--(2.758,.011)--cycle;
\filldraw[fill=white](.177,.321)--(.273,.606)--(.065,.249)--(-.035,-.019)--cycle;
\filldraw[fill=gray,fill opacity=0.5,draw=none](2.37,-.326)--(2.329,-.314)--(2.256,-.275)--(2.204,-.225)--(2.178,-.169)--(2.181,-.113)--(2.196,-.09)--cycle;
\draw[draw=gray!50!black,draw opacity=0.5](2.37,-.326)--(2.329,-.314)--(2.256,-.275)--(2.204,-.225)--(2.178,-.169)--(2.181,-.113)--(2.196,-.09);
\draw(2.049,-.234)--(.268,.585);
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.178,-.169)--(2.19,-.049)--(2.194,.007)--(2.181,-.113)--cycle;
\draw[color=gray](2.654,-.646)--(2.589,-.669);
\filldraw[fill=gray,draw=none](2.644,-.717)--(3.604,-.513)--(3.56,-.452)--(2.599,-.657)--cycle;
\draw(2.644,-.717)--(3.604,-.513)--(3.56,-.452)--(2.599,-.657);
\filldraw[fill=gray,draw=none](3.295,-.661)--(3.595,-.597)--(3.604,-.513)--(3.304,-.576)--cycle;
\draw(3.295,-.661)--(3.595,-.597)--(3.604,-.513)--(3.304,-.576);
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.818,-.415)--(3.844,-.471)--(3.84,-.526)--(3.808,-.577)--(3.751,-.617)--(3.673,-.644)--(3.583,-.653)--(3.49,-.645)--(3.402,-.62)--(3.328,-.58)--(3.276,-.53)--(3.25,-.475)--(3.254,-.419)--(3.286,-.368)--(3.343,-.328)--(3.421,-.302)--(3.511,-.292)--(3.604,-.3)--(3.692,-.325)--(3.766,-.365)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.511,-.292)--(3.523,-.172)--(3.617,-.181)--(3.604,-.3)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.604,-.3)--(3.617,-.181)--(3.705,-.206)--(3.692,-.325)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.421,-.302)--(3.433,-.182)--(3.523,-.172)--(3.511,-.292)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.768,-.221)--(2.78,-.101)--(2.748,-.151)--(2.736,-.271)--cycle;
\filldraw[fill=gray](2.531,-.026)--(2.516,-.018)--(2.498,-.013)--(2.48,-.011)--(2.462,-.013)--(2.446,-.018)--(2.435,-.026)--(2.428,-.036)--(2.428,-.048)--(2.433,-.059)--(2.443,-.069)--(2.458,-.077)--(2.476,-.082)--(2.494,-.083)--(2.512,-.081)--(2.528,-.076)--(2.539,-.068)--(2.546,-.058)--(2.546,-.047)--(2.541,-.036)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.204,-.225)--(2.216,-.105)--(2.19,-.049)--(2.178,-.169)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.692,-.325)--(3.705,-.206)--(3.778,-.245)--(3.766,-.365)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.343,-.328)--(3.356,-.208)--(3.433,-.182)--(3.421,-.302)--cycle;
\draw[color=gray](2.698,-.568)--(2.335,-.506);
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.766,-.365)--(3.778,-.245)--(3.83,-.295)--(3.818,-.415)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.286,-.368)--(3.298,-.248)--(3.356,-.208)--(3.343,-.328)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.736,-.271)--(2.748,-.151)--(2.691,-.192)--(2.678,-.312)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.818,-.415)--(3.83,-.295)--(3.856,-.351)--(3.844,-.471)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.254,-.419)--(3.266,-.299)--(3.298,-.248)--(3.286,-.368)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.844,-.471)--(3.856,-.351)--(3.853,-.407)--(3.84,-.526)--cycle;
\filldraw[fill=gray](3.488,-.473)--(3.5,-.353)--(3.501,-.342)--(3.488,-.462)--cycle;
\filldraw[fill=gray](3.606,-.483)--(3.618,-.364)--(3.612,-.374)--(3.599,-.493)--cycle;
\filldraw[fill=gray](3.493,-.484)--(3.505,-.364)--(3.5,-.353)--(3.488,-.473)--cycle;
\filldraw[fill=gray](3.599,-.493)--(3.612,-.374)--(3.6,-.382)--(3.588,-.502)--cycle;
\filldraw[fill=gray](3.503,-.494)--(3.516,-.374)--(3.505,-.364)--(3.493,-.484)--cycle;
\filldraw[fill=gray](3.588,-.502)--(3.6,-.382)--(3.585,-.387)--(3.572,-.507)--cycle;
\filldraw[fill=gray](3.518,-.502)--(3.53,-.382)--(3.516,-.374)--(3.503,-.494)--cycle;
\filldraw[fill=gray](3.603,-.331)--(3.588,-.323)--(3.571,-.318)--(3.552,-.317)--(3.534,-.319)--(3.519,-.324)--(3.507,-.332)--(3.501,-.342)--(3.5,-.353)--(3.505,-.364)--(3.516,-.374)--(3.53,-.382)--(3.548,-.387)--(3.567,-.389)--(3.585,-.387)--(3.6,-.382)--(3.612,-.374)--(3.618,-.364)--(3.619,-.352)--(3.614,-.341)--cycle;
\filldraw[fill=gray](3.572,-.507)--(3.585,-.387)--(3.567,-.389)--(3.554,-.509)--cycle;
\filldraw[fill=gray](3.536,-.507)--(3.548,-.387)--(3.53,-.382)--(3.518,-.502)--cycle;
\filldraw[fill=gray](3.554,-.509)--(3.567,-.389)--(3.548,-.387)--(3.536,-.507)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.778,-.245)--(3.705,-.206)--(3.617,-.181)--(3.523,-.172)--(3.433,-.182)--(3.356,-.208)--(3.298,-.248)--(3.266,-.299)--(3.263,-.355)--(3.288,-.41)--(3.34,-.46)--(3.414,-.5)--(3.502,-.525)--(3.595,-.533)--(3.685,-.524)--(3.763,-.497)--(3.821,-.457)--(3.853,-.407)--(3.856,-.351)--(3.83,-.295)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.256,-.275)--(2.268,-.155)--(2.216,-.105)--(2.204,-.225)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.678,-.312)--(2.691,-.192)--(2.613,-.218)--(2.601,-.338)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.329,-.314)--(2.342,-.194)--(2.268,-.155)--(2.256,-.275)--cycle;
\filldraw[fill=gray,draw=none](2.635,-.802)--(3.295,-.661)--(3.304,-.576)--(2.644,-.717)--cycle;
\draw(2.635,-.802)--(3.295,-.661);
\draw(3.304,-.576)--(2.644,-.717);
\draw(2.745,-.554)--(2.523,-.452);
\draw[arrows=-,line width=2pt,color=blue](2.749,-.569)--(2.538,-.508);
\draw[arrows=-,line width=.4pt,color=blue](2.749,-.569)--(2.538,-.508);
\draw[color=gray](2.704,-.629)--(2.654,-.646);
\filldraw[fill=white](2.706,-.85)--(2.725,-.67)--(2.546,-.429)--(2.528,-.608)--cycle;
\draw[color=gray](2.589,-.669)--(-.625,-1.795);
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.601,-.338)--(2.613,-.218)--(2.523,-.228)--(2.511,-.347)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.417,-.339)--(2.43,-.219)--(2.342,-.194)--(2.329,-.314)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.25,-.475)--(3.263,-.355)--(3.266,-.299)--(3.254,-.419)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.511,-.347)--(2.523,-.228)--(2.43,-.219)--(2.417,-.339)--cycle;
\draw[color=gray](2.488,-.161)--(2.019,.445);
\draw[arrows=-latex,line width=2pt,color=blue](2.538,-.508)--(1.415,-.188);
\draw[arrows=-latex,line width=.4pt,color=blue](2.538,-.508)--(1.415,-.188);
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.84,-.526)--(3.853,-.407)--(3.821,-.457)--(3.808,-.577)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.276,-.53)--(3.288,-.41)--(3.263,-.355)--(3.25,-.475)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.808,-.577)--(3.821,-.457)--(3.763,-.497)--(3.751,-.617)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.328,-.58)--(3.34,-.46)--(3.288,-.41)--(3.276,-.53)--cycle;
\draw(2.523,-.452)--(2.049,-.234);
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.751,-.617)--(3.763,-.497)--(3.685,-.524)--(3.673,-.644)--cycle;
\draw[color=gray](2.819,-.589)--(2.703,-.569);
\draw[color=gray](2.819,-.589)--(2.674,-.401);
\draw[arrows=-,line width=2pt,color=Maroon1](2.819,-.589)--(2.819,-.648);
\draw(2.819,-.589)--(2.745,-.554);
\draw[arrows=-,line width=.4pt,color=blue](2.819,-.589)--(2.749,-.569);
\draw[arrows=-,line width=2pt,color=blue](2.819,-.589)--(2.749,-.569);
\draw[color=gray](2.762,-.609)--(2.704,-.629);
\draw[color=gray](2.819,-.589)--(2.762,-.609);
\draw[color=gray](2.819,-.589)--(2.766,-.569);
\draw[arrows=-,line width=.4pt,color=red](2.819,-.589)--(2.793,-.629);
\draw[arrows=-,line width=2pt,color=red](2.819,-.589)--(2.793,-.629);
\draw[arrows=-,line width=.4pt,color=green](2.819,-.589)--(2.827,-.509);
\draw[arrows=-,line width=2pt,color=green](2.819,-.589)--(2.827,-.509);
\draw[color=gray](2.766,-.569)--(2.606,-.509);
\draw[arrows=-,line width=2pt,color=red](2.793,-.629)--(2.716,-.75);
\draw[arrows=-,line width=.4pt,color=red](2.793,-.629)--(2.716,-.75);
\filldraw[fill=white](2.546,-.429)--(2.725,-.67)--(3.108,-.589)--(2.93,-.347)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.402,-.62)--(3.414,-.5)--(3.34,-.46)--(3.328,-.58)--cycle;
\draw[color=gray](2.674,-.401)--(2.488,-.161);
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.673,-.644)--(3.685,-.524)--(3.595,-.533)--(3.583,-.653)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.49,-.645)--(3.502,-.525)--(3.414,-.5)--(3.402,-.62)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.583,-.653)--(3.595,-.533)--(3.502,-.525)--(3.49,-.645)--cycle;
\filldraw[fill=white,draw=none](2.854,-.777)--(2.85,-.819)--(3.09,-.768)--(3.094,-.726)--cycle;
\draw(2.85,-.819)--(3.09,-.768)--(3.094,-.726);
\filldraw[fill=gray,draw=none](2.779,-.771)--(3.114,-1.226)--(3.123,-1.141)--(2.788,-.686)--cycle;
\draw(2.779,-.771)--(3.114,-1.226)--(3.123,-1.141)--(2.788,-.686);
\filldraw[fill=gray,draw=none](2.788,-.686)--(3.123,-1.141)--(3.218,-1.12)--(2.883,-.666)--cycle;
\draw(2.788,-.686)--(3.123,-1.141)--(3.218,-1.12)--(2.883,-.666);
\filldraw[fill=gray,draw=none](2.067,-.84)--(2.644,-.717)--(2.599,-.657)--(2.022,-.779)--cycle;
\draw(2.599,-.657)--(2.022,-.779)--(2.067,-.84)--(2.644,-.717);
\filldraw[fill=gray,draw=none](2.058,-.925)--(2.635,-.802)--(2.644,-.717)--(2.067,-.84)--cycle;
\draw(2.644,-.717)--(2.067,-.84)--(2.058,-.925)--(2.635,-.802);
\filldraw[fill=white,draw=none](2.854,-.777)--(3.094,-.726)--(3.108,-.589)--(2.868,-.64)--cycle;
\draw(3.094,-.726)--(3.108,-.589)--(2.868,-.64);
\filldraw[fill=gray](2.067,-.84)--(2.022,-.779)--(2.014,-.864)--(2.058,-.925)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.354,-.727)--(2.38,-.782)--(2.376,-.838)--(2.344,-.889)--(2.287,-.929)--(2.209,-.955)--(2.119,-.965)--(2.026,-.957)--(1.938,-.932)--(1.864,-.892)--(1.812,-.842)--(1.786,-.786)--(1.789,-.731)--(1.822,-.68)--(1.879,-.64)--(1.957,-.613)--(2.047,-.604)--(2.14,-.612)--(2.228,-.637)--(2.302,-.677)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.047,-.604)--(2.059,-.484)--(2.153,-.492)--(2.14,-.612)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.14,-.612)--(2.153,-.492)--(2.24,-.517)--(2.228,-.637)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](1.957,-.613)--(1.969,-.494)--(2.059,-.484)--(2.047,-.604)--cycle;
\draw[arrows=-latex,line width=2pt,color=blue](-4.358,-2.656)--(-3.845,-1.848);
\draw[arrows=-latex,line width=2pt,color=green](2.827,-.509)--(2.942,.61);
\draw[arrows=-latex,line width=.4pt,color=green](2.827,-.509)--(2.942,.61);
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.228,-.637)--(2.24,-.517)--(2.314,-.557)--(2.302,-.677)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](1.879,-.64)--(1.892,-.52)--(1.969,-.494)--(1.957,-.613)--cycle;
\draw[color=gray](2.606,-.509)--(-.379,.602);
\filldraw[fill=white,draw=none](2.85,-.819)--(2.854,-.777)--(2.711,-.808)--(2.706,-.85)--cycle;
\draw(2.711,-.808)--(2.706,-.85)--(2.85,-.819);
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.302,-.677)--(2.314,-.557)--(2.366,-.607)--(2.354,-.727)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](1.822,-.68)--(1.834,-.56)--(1.892,-.52)--(1.879,-.64)--cycle;
\filldraw[fill=white,draw=none](2.854,-.777)--(2.868,-.64)--(2.725,-.67)--(2.711,-.808)--cycle;
\draw(2.868,-.64)--(2.725,-.67)--(2.711,-.808);
\filldraw[fill=gray,fill opacity=0.5,draw=none](2.369,-.758)--(2.354,-.727)--(2.366,-.607)--(2.381,-.639)--cycle;
\draw[draw=gray!50!black,draw opacity=0.5](2.369,-.758)--(2.354,-.727)--(2.366,-.607)--(2.381,-.639);
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](1.789,-.731)--(1.802,-.611)--(1.834,-.56)--(1.822,-.68)--cycle;
\filldraw[fill=gray,fill opacity=0.5,draw=none](2.369,-.758)--(2.381,-.639)--(2.392,-.662)--(2.38,-.782)--cycle;
\draw[draw=gray!50!black,draw opacity=0.5](2.381,-.639)--(2.392,-.662)--(2.38,-.782)--(2.369,-.758);
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.38,-.782)--(2.392,-.662)--(2.389,-.718)--(2.376,-.838)--cycle;
\filldraw[fill=gray](2.024,-.785)--(2.036,-.665)--(2.037,-.654)--(2.024,-.774)--cycle;
\filldraw[fill=gray](2.142,-.795)--(2.154,-.675)--(2.147,-.685)--(2.135,-.805)--cycle;
\filldraw[fill=gray](2.029,-.796)--(2.041,-.676)--(2.036,-.665)--(2.024,-.785)--cycle;
\filldraw[fill=gray](2.135,-.805)--(2.147,-.685)--(2.136,-.693)--(2.124,-.813)--cycle;
\filldraw[fill=gray](2.039,-.806)--(2.051,-.686)--(2.041,-.676)--(2.029,-.796)--cycle;
\filldraw[fill=gray](2.124,-.813)--(2.136,-.693)--(2.12,-.699)--(2.108,-.819)--cycle;
\filldraw[fill=gray](2.054,-.814)--(2.066,-.694)--(2.051,-.686)--(2.039,-.806)--cycle;
\filldraw[fill=gray](2.108,-.819)--(2.12,-.699)--(2.102,-.701)--(2.09,-.82)--cycle;
\filldraw[fill=gray](2.071,-.819)--(2.084,-.699)--(2.066,-.694)--(2.054,-.814)--cycle;
\filldraw[fill=gray](2.09,-.82)--(2.102,-.701)--(2.084,-.699)--(2.071,-.819)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.314,-.557)--(2.24,-.517)--(2.153,-.492)--(2.059,-.484)--(1.969,-.494)--(1.892,-.52)--(1.834,-.56)--(1.802,-.611)--(1.798,-.667)--(1.824,-.722)--(1.876,-.772)--(1.95,-.812)--(2.038,-.837)--(2.131,-.845)--(2.221,-.835)--(2.299,-.809)--(2.357,-.769)--(2.389,-.718)--(2.392,-.662)--(2.366,-.607)--cycle;
\draw[arrows=-latex,line width=2pt,color=red](2.716,-.75)--(2.306,-1.397);
\draw[arrows=-latex,line width=.4pt,color=red](2.716,-.75)--(2.306,-1.397);
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](1.786,-.786)--(1.798,-.667)--(1.802,-.611)--(1.789,-.731)--cycle;
\filldraw[fill=gray](3.114,-1.226)--(3.21,-1.205)--(3.218,-1.12)--(3.123,-1.141)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.426,-1.032)--(3.452,-1.088)--(3.449,-1.144)--(3.417,-1.194)--(3.359,-1.235)--(3.281,-1.261)--(3.191,-1.27)--(3.098,-1.262)--(3.01,-1.237)--(2.936,-1.198)--(2.884,-1.148)--(2.858,-1.092)--(2.862,-1.036)--(2.894,-.986)--(2.952,-.945)--(3.029,-.919)--(3.119,-.91)--(3.213,-.918)--(3.301,-.943)--(3.374,-.982)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.119,-.91)--(3.131,-.79)--(3.225,-.798)--(3.213,-.918)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.213,-.918)--(3.225,-.798)--(3.313,-.823)--(3.301,-.943)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.029,-.919)--(3.042,-.799)--(3.131,-.79)--(3.119,-.91)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.376,-.838)--(2.389,-.718)--(2.357,-.769)--(2.344,-.889)--cycle;
\filldraw[fill=gray](2.139,-.643)--(2.124,-.635)--(2.107,-.63)--(2.088,-.628)--(2.07,-.63)--(2.054,-.636)--(2.043,-.644)--(2.037,-.654)--(2.036,-.665)--(2.041,-.676)--(2.051,-.686)--(2.066,-.694)--(2.084,-.699)--(2.102,-.701)--(2.12,-.699)--(2.136,-.693)--(2.147,-.685)--(2.154,-.675)--(2.155,-.664)--(2.149,-.653)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](1.812,-.842)--(1.824,-.722)--(1.798,-.667)--(1.786,-.786)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.301,-.943)--(3.313,-.823)--(3.386,-.862)--(3.374,-.982)--cycle;
\filldraw[fill=gray,fill opacity=0.5,draw=none](2.985,-.934)--(2.997,-.814)--(3.042,-.799)--(3.029,-.919)--cycle;
\draw[draw=gray!50!black,draw opacity=0.5](2.997,-.814)--(3.042,-.799)--(3.029,-.919)--(2.985,-.934);
\draw[arrows=-latex,line width=2pt,color=Maroon1](-4.358,-2.656)--(-4.358,-3.885);
\filldraw[fill=gray,fill opacity=0.5,draw=none](2.985,-.934)--(2.952,-.945)--(2.964,-.825)--(2.997,-.814)--cycle;
\draw[draw=gray!50!black,draw opacity=0.5](2.985,-.934)--(2.952,-.945)--(2.964,-.825)--(2.997,-.814);
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.374,-.982)--(3.386,-.862)--(3.439,-.912)--(3.426,-1.032)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.894,-.986)--(2.906,-.866)--(2.964,-.825)--(2.952,-.945)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.344,-.889)--(2.357,-.769)--(2.299,-.809)--(2.287,-.929)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.426,-1.032)--(3.439,-.912)--(3.464,-.968)--(3.452,-1.088)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.862,-1.036)--(2.874,-.916)--(2.906,-.866)--(2.894,-.986)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.452,-1.088)--(3.464,-.968)--(3.461,-1.024)--(3.449,-1.144)--cycle;
\filldraw[fill=gray](3.096,-1.09)--(3.108,-.971)--(3.109,-.959)--(3.097,-1.079)--cycle;
\filldraw[fill=gray](3.214,-1.101)--(3.226,-.981)--(3.22,-.991)--(3.208,-1.111)--cycle;
\filldraw[fill=gray](3.101,-1.102)--(3.113,-.982)--(3.108,-.971)--(3.096,-1.09)--cycle;
\filldraw[fill=gray](3.208,-1.111)--(3.22,-.991)--(3.208,-.999)--(3.196,-1.119)--cycle;
\filldraw[fill=gray](3.111,-1.112)--(3.124,-.992)--(3.113,-.982)--(3.101,-1.102)--cycle;
\filldraw[fill=gray](3.196,-1.119)--(3.208,-.999)--(3.193,-1.004)--(3.18,-1.124)--cycle;
\filldraw[fill=gray](3.126,-1.119)--(3.138,-1)--(3.124,-.992)--(3.111,-1.112)--cycle;
\filldraw[fill=gray](3.18,-1.124)--(3.193,-1.004)--(3.175,-1.006)--(3.162,-1.126)--cycle;
\filldraw[fill=gray](3.144,-1.124)--(3.156,-1.005)--(3.138,-1)--(3.126,-1.119)--cycle;
\filldraw[fill=gray](3.162,-1.126)--(3.175,-1.006)--(3.156,-1.005)--(3.144,-1.124)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.386,-.862)--(3.313,-.823)--(3.225,-.798)--(3.131,-.79)--(3.042,-.799)--(2.964,-.825)--(2.906,-.866)--(2.874,-.916)--(2.871,-.972)--(2.896,-1.028)--(2.949,-1.078)--(3.022,-1.117)--(3.11,-1.142)--(3.204,-1.151)--(3.294,-1.141)--(3.371,-1.115)--(3.429,-1.075)--(3.461,-1.024)--(3.464,-.968)--(3.439,-.912)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](1.864,-.892)--(1.876,-.772)--(1.824,-.722)--(1.812,-.842)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.287,-.929)--(2.299,-.809)--(2.221,-.835)--(2.209,-.955)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](1.938,-.932)--(1.95,-.812)--(1.876,-.772)--(1.864,-.892)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.209,-.955)--(2.221,-.835)--(2.131,-.845)--(2.119,-.965)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.026,-.957)--(2.038,-.837)--(1.95,-.812)--(1.938,-.932)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.858,-1.092)--(2.871,-.972)--(2.874,-.916)--(2.862,-1.036)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.119,-.965)--(2.131,-.845)--(2.038,-.837)--(2.026,-.957)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.449,-1.144)--(3.461,-1.024)--(3.429,-1.075)--(3.417,-1.194)--cycle;
\filldraw[fill=gray](3.211,-.949)--(3.197,-.941)--(3.179,-.936)--(3.16,-.934)--(3.142,-.936)--(3.127,-.941)--(3.115,-.949)--(3.109,-.959)--(3.108,-.971)--(3.113,-.982)--(3.124,-.992)--(3.138,-1)--(3.156,-1.005)--(3.175,-1.006)--(3.193,-1.004)--(3.208,-.999)--(3.22,-.991)--(3.226,-.981)--(3.227,-.97)--(3.222,-.959)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.884,-1.148)--(2.896,-1.028)--(2.871,-.972)--(2.858,-1.092)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.417,-1.194)--(3.429,-1.075)--(3.371,-1.115)--(3.359,-1.235)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](2.936,-1.198)--(2.949,-1.078)--(2.896,-1.028)--(2.884,-1.148)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.359,-1.235)--(3.371,-1.115)--(3.294,-1.141)--(3.281,-1.261)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.01,-1.237)--(3.022,-1.117)--(2.949,-1.078)--(2.936,-1.198)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.281,-1.261)--(3.294,-1.141)--(3.204,-1.151)--(3.191,-1.27)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.098,-1.262)--(3.11,-1.142)--(3.022,-1.117)--(3.01,-1.237)--cycle;
\filldraw[fill=gray,draw=gray!50!black,fill opacity=0.5,draw opacity=0.5](3.191,-1.27)--(3.204,-1.151)--(3.11,-1.142)--(3.098,-1.262)--cycle;
\draw[arrows=-latex,line width=2pt,color=red](-4.358,-2.656)--(-5.768,-2.362);
\draw[arrows=-latex,line width=2pt,color=green](-4.358,-2.656)--(-4.358,-1.427);
 \path (-4.358,-2.656) -- (-5.768,-2.362) node[pos=1.25] {$x$};  \path (-4.358,-2.656) -- (-4.358,-1.427) node[pos=1.25] {$y$};  \path (-4.358,-2.656) -- (-3.845,-1.848) node[pos=1.25] {$z$};  \coordinate (pAbsolute) at (-4.358,-2.656);  \coordinate (pBody) at (2.819,-.589);  \coordinate (pHouse) at (-3.792,2.452);  \coordinate (pHouseProject) at (.273,.606);  \coordinate (pGravity) at (-4.358,-3.885);  \coordinate (pGravityBody) at (2.819,-1.817); % End sketch output


==> figures/tikz/notation.tex <==
  \begin{tikzpicture}[p/.style={inner sep=0pt, minimum size=3pt, circle, fill=black},l/.style={fill=white}]
    \input{figures/sketch/imu_quadrotor_image}
    \draw (pAbsolute) edge[out=2,in=-135, thick,latex-, shorten >=8mm, shorten <=8mm] (pBody);
    \node[anchor=north west,text width=5cm] at ($(pAbsolute) + (4.5,0.2)$) {$R_f$, $T_f$: transformation\\ from $\cR_f$ to $\cR_s$};
    \node[anchor=south west, text width=10cm] at (pHouse) {$X_{sp}$: 3-D point expressed in $\cR_s$, $p\in\{1,\ldots, P\}$\\$X_{cfp}$:   3-D point expressed in $\cR_f$};
    \node[p] at (pHouse) {};
    \node[anchor=north west] at (pAbsolute) {$\cR_s$: absolute reference};
    \node[anchor=west, text width=4cm] at ($(pBody)+(1.3,0.8)$) {$\cR_f$: body reference\\ at frame $f\in \{1,\ldots,F\}$\\\medskip$\tau_f$, $\nu_f$, $\omega_f$: translation, \\velocity, and angular\\ velocity in $\cR_f$};
    \node[l,anchor=south west] at (pHouseProject) {$x_{fp}$: image of $X_{cfp}$};
    \node[p] at (pHouseProject) {};
    \node[text width=5cm] at (5,3) {}; 
    \node[anchor=west] at ($(pGravity)+(0,0.1)$) {$g_s$: gravity vector in $\cR_s$};
    \node[anchor=west] at ($(pGravityBody)+(0,0.1)$) {$\alpha_{IMU}$: acceleration from IMU};
  \end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../2016-cvpr-dynamicSfM"
%%% End:


==> preamble/common.tex <==
\input{preamble/commonNoTikz}
\input{preamble/graphicsTikz}

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/compactLists.tex <==
% set compact lists
\setlist[1]{\labelindent=\parindent}
\setlist[1]{topsep=3pt, itemsep=0pt}


==> preamble/graphLocalization.tex <==
% This file was generated by the scriptgenerateGraphLocalization
% Do not modify this file directly

% Notation for nodes
\newcommand{\Ri}{R_{i}}
\newcommand{\dRi}{\dot{R}_{i}}
\newcommand{\ddRi}{\ddot{R}_{i}}
\newcommand{\Ti}{T_{i}}
\newcommand{\dTi}{\dot{T}_{i}}
\newcommand{\ddTi}{\ddot{T}_{i}}

\newcommand{\Rj}{R_{j}}
\newcommand{\dRj}{\dot{R}_{j}}
\newcommand{\ddRj}{\ddot{R}_{j}}
\newcommand{\Tj}{T_{j}}
\newcommand{\dTj}{\dot{T}_{j}}
\newcommand{\ddTj}{\ddot{T}_{j}}


% Notation for edges
\newcommand{\Rij}{R_{ij}}
\newcommand{\Tij}{T_{ij}}
\newcommand{\betaij}{\beta_{ij}}
\newcommand{\cij}{c_{ij}}
\newcommand{\dij}{d_{ij}}
\newcommand{\qij}{q_{ij}}
\newcommand{\lij}{\lambda_{ij}}
\newcommand{\varphiij}{\varphi_{ij}}
\newcommand{\gij}{g_{ij}}

\newcommand{\Rji}{R_{ji}}
\newcommand{\Tji}{T_{ji}}
\newcommand{\betaji}{\beta_{ji}}
\newcommand{\cji}{c_{ji}}
\newcommand{\dji}{d_{ji}}
\newcommand{\qji}{q_{ji}}
\newcommand{\lji}{\lambda_{ji}}
\newcommand{\varphiji}{\varphi_{ji}}
\newcommand{\gji}{g_{ji}}


% Notation for edges, measured quantities
\newcommand{\tRij}{\tilde{R}_{ij}}
\newcommand{\dtRij}{\dot{\tilde{R}}_{ij}}
\newcommand{\tTij}{\tilde{T}_{ij}}
\newcommand{\dtTij}{\dot{\tilde{T}}_{ij}}
\newcommand{\tbetaij}{\tilde{\beta}_{ij}}
\newcommand{\dtbetaij}{\dot{\tilde{\beta}}_{ij}}
\newcommand{\tcij}{\tilde{c}_{ij}}
\newcommand{\dtcij}{\dot{\tilde{c}}_{ij}}
\newcommand{\tdij}{\tilde{d}_{ij}}
\newcommand{\dtdij}{\dot{\tilde{d}}_{ij}}
\newcommand{\tqij}{\tilde{q}_{ij}}
\newcommand{\dtqij}{\dot{\tilde{q}}_{ij}}
\newcommand{\tlij}{\tilde{\lambda}_{ij}}
\newcommand{\dtlij}{\dot{\tilde{\lambda}}_{ij}}
\newcommand{\tvarphiij}{\tilde{\varphi}_{ij}}
\newcommand{\dtvarphiij}{\dot{\tilde{\varphi}}_{ij}}
\newcommand{\tgij}{\tilde{g}_{ij}}
\newcommand{\dtgij}{\dot{\tilde{g}}_{ij}}

\newcommand{\tRji}{\tilde{R}_{ji}}
\newcommand{\dtRji}{\dot{\tilde{R}}_{ji}}
\newcommand{\tTji}{\tilde{T}_{ji}}
\newcommand{\dtTji}{\dot{\tilde{T}}_{ji}}
\newcommand{\tbetaji}{\tilde{\beta}_{ji}}
\newcommand{\dtbetaji}{\dot{\tilde{\beta}}_{ji}}
\newcommand{\tcji}{\tilde{c}_{ji}}
\newcommand{\dtcji}{\dot{\tilde{c}}_{ji}}
\newcommand{\tdji}{\tilde{d}_{ji}}
\newcommand{\dtdji}{\dot{\tilde{d}}_{ji}}
\newcommand{\tqji}{\tilde{q}_{ji}}
\newcommand{\dtqji}{\dot{\tilde{q}}_{ji}}
\newcommand{\tlji}{\tilde{\lambda}_{ji}}
\newcommand{\dtlji}{\dot{\tilde{\lambda}}_{ji}}
\newcommand{\tvarphiji}{\tilde{\varphi}_{ji}}
\newcommand{\dtvarphiji}{\dot{\tilde{\varphi}}_{ji}}
\newcommand{\tgji}{\tilde{g}_{ji}}
\newcommand{\dtgji}{\dot{\tilde{g}}_{ji}}


% Node state differences
\newcommand{\xjmi}{x_j-x_i}
\newcommand{\vjmi}{v_j-v_i}
\newcommand{\nxjmi}{\norm{\xjmi}}

% Notation for desired quantities
\newcommand{\xgi}{x_{g,i}}
\newcommand{\xgj}{x_{g,j}}
\newcommand{\betagij}{\beta_{g,ij}}
\newcommand{\dgij}{d_{g,ij}}


==> preamble/graphicsExport.tex <==
% activate externalization of figures
\usetikzlibrary{external}

\tikzexternalize 

%command to insert a Beamer frame from a sketch and externalize with the same name 
\newcommand{\insertsketchframe}[1]{\section{$\mathrm{#1}$}%
\tikzsetnextfilename{#1}%
  \begin{tikzpicture}[scale=0.7]%
    \input{sketch/#1}%
  \end{tikzpicture}%
\endpgfgraphicnamed%
}

%command to insert a Beamer frame from a tikz drawing and externalize with the same name 
\newcommand{\inserttikzframe}[1]{\section{$\mathrm{#1}$}%
\tikzsetnextfilename{#1}%
\input{tikz/#1}%
\endpgfgraphicnamed%
}


==> preamble/graphicsTikz.tex <==
%TikZ and common libraries
\usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{matrix}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{arrows.meta}

%Draw normalized vector between two coordinates
\newcommand\normalize[2][(0,0)]{%
  \draw[blue,->] (#1) -- ($(#1)!1cm!(#2)$) coordinate (#1#2norm)}

%Quotatures
\tikzset{
  dim above/.style={to path={\pgfextra{
        \pgfinterruptpath
        \draw[>=latex,|->|] let
        \p1=($(\tikztostart)!3mm!90:(\tikztotarget)$),
        \p2=($(\tikztotarget)!3mm!-90:(\tikztostart)$)
        in(\p1) -- (\p2) node[pos=.5,sloped,above]{#1};
        \endpgfinterruptpath
      }
    }
  },
  dim double above/.style={to path={\pgfextra{
        \pgfinterruptpath
        \draw[>=latex,|->|] let
        \p1=($(\tikztostart)!8mm!90:(\tikztotarget)$),
        \p2=($(\tikztotarget)!8mm!-90:(\tikztostart)$)
        in(\p1) -- (\p2) node[pos=.5,sloped,above]{#1};
        \endpgfinterruptpath
      }
    }
  },
  dim below/.style={to path={\pgfextra{
        \pgfinterruptpath
        \draw[>=latex,|->|] let 
        \p1=($(\tikztostart)!6mm!-90:(\tikztotarget)$),
        \p2=($(\tikztotarget)!6mm!90:(\tikztostart)$)
        in (\p1) -- (\p2) node[pos=.5,sloped,below]{#1};
        \endpgfinterruptpath
      }
    }
  },
}

%Horizontally fit an image between two coordinates
\newcommand{\imageBetween}[3]{\draw (#2) let \p1 = ($ (#3) - (#2) $) in node[inner sep=0pt,anchor=south west, text width={veclen(\x1,\y1)}] {\includegraphics[width=\linewidth]{#1}};}


==> preamble/posterCommon.tex <==
\input{preamble/posterGraphics}
\input{preamble/posterFormatting}

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> preamble/posterFormatting.tex <==
%fonts
\usepackage[scaled=0.90]{helvet}
\usepackage{courier}

%sectioning
\pagestyle{empty}
\setcounter{secnumdepth}{0}

%headings
\def\Head#1{\noindent\hbox to \hsize{\hfil{\veryHuge\color{DarkBlue} #1}}\bigskip}
\def\LHead#1{\noindent{\LARGE\color{Blue} #1}\vspace{-.5cm}}
\def\Subhead#1{\noindent{\Large\color{DarkBlue} #1}\vspace{-.5cm}}
\def\Subsubhead#1{{\color{Blue} #1}}
\def\Title#1{\noindent{\Huge #1}}

%text boxes and grid
%Note: use options showboxes if you want to see the boxes
\usepackage[absolute]{textpos}
\TPGrid[30mm,30mm]{10}{20}  % 3 - 1 - 7 - 1 - 3 Columns

% Mess with these as you like
\parindent=0pt
%\parindent=1cm
\parskip=0.5\baselineskip


==> preamble/posterGraphics.tex <==
\usepackage{tikz}
\usepackage{xcolor}

%colors
\definecolor{Blue}{rgb}{0.05,0.2,0.5}
\definecolor{DarkBlue}{rgb}{0.1,0.1,0.5}
\definecolor{LightBlue}{rgb}{.2431,.5451,.8588}
\definecolor{Red}{rgb}{1.0,0,0}
\definecolor{LightGray}{rgb}{0.95,0.95,0.95}

%for callouts
\usetikzlibrary{calc,chains,positioning,shapes.callouts}

%bullet points
\renewcommand{\labelitemi}{\color{LightBlue}{$\bullet$}}

%highlighting
\newcommand{\alert}[1]{{\color{LightBlue} #1}}

%rounded boxes
\newenvironment{roundboxes}[1][]
{\begin{tikzpicture}[start chain,node distance=2cm,
 every node/.style={on chain, text=black,fill=LightBlue!20, rounded corners=0.6cm},#1]
}
{\end{tikzpicture}
}

%Define anchors for callouts
\newcommand{\anchor}[1]{\tikz[remember picture] \coordinate (#1);}

%Insert callouts. Syntax:
%\callout[optionalStyle]{pointer}{positionRelativeToThePointer}{text}
\newcommand{\callout}[4][]{\begin{tikzpicture}[remember picture, overlay]
 \node[rectangle callout, fill=gray!50, #1, callout absolute pointer={#2}] at ($ #2 + #3 $) {#4};
\end{tikzpicture}
}

%Rounded box to highlight plus define anchor
\newcommand{\enboxref}[3][]{
  \tikz[baseline,remember picture]{
    \node[fill=gray!20,anchor=base,rounded corners=0.6cm,#1] (#2) {#3};
  }
}

%Boxes to define sections
\newlength{\sectionboxpadding}
\setlength{\sectionboxpadding}{5mm}

\newcommand{\sectionboxcolor}{LightBlue}

\newcommand{\sectionboxstart}[1]{\makebox[0cm][l]{\anchor{#1 a}}}
\newcommand{\sectionboxend}[1]{\makebox[0cm][l]{\anchor{#1 b}} \vspace{-3em}\\}
\newcommand{\sectionboxdraw}[2][]{\begin{tikzpicture}[remember picture, overlay,#1]
 \draw[rounded corners, line width=5pt, draw=\sectionboxcolor] ($(#2 a)+(0,0.6em)+(-\sectionboxpadding,\sectionboxpadding)+(0,0.4em)$) rectangle ($(#2 b)+(\textwidth,1em)+(\sectionboxpadding,-\sectionboxpadding)+(0,0.4em)$);
\end{tikzpicture}
}

\newcommand{\generalboxdraw}{
\begin{tikzpicture}[remember picture, overlay, LightBlue]
\draw[line width=5pt] ($(current page.north west) + (2,-13.5)$) rectangle ($(current page.south east) + (-2,3)$);
\end{tikzpicture}
}


==> preamble/proposals.tex <==
\input{preamble/compactLists}
\usepackage{url}
\usepackage{times}
\usepackage[compact]{titlesec}

%reduce line skip before \paragraph
\titlespacing{\paragraph}{%
  0pt}{%              left margin
  0\baselineskip}{% space before (vertical)
  0.5em}%               space after (horizontal)

\newcommand{\testgrid}{\tikz[remember picture, overlay]{%
  \coordinate (tl) at  ($(current page.north west)+(1in,-1in)$);%
  \coordinate (br) at  ($(current page.south east)+(-1in,1in)$);%
  \draw[red] (tl) rectangle (br);%
  \draw[red] (tl) grid[xstep=2\textwidth,ystep=1in] (br);}}


%Perfect 1 inch margins
\usepackage[letterpaper,margin=1in]{geometry}

%Make font for captions smaller (saves space and visually separates them from the main text)
\usepackage[font=footnotesize]{caption}

\input{preamble/proposalsFormatting}
\input{preamble/proposalsSplitting}


==> preamble/proposalsAggressive.tex <==
\linespread{0.93}


==> preamble/proposalsFormatting.tex <==
%Make an enumeration with a letter+progressive number
\newenvironment{lenumerate}[1]
{\begin{enumerate}[label=(#1\arabic*),leftmargin=0.2in,itemindent=0.15in]}
{\end{enumerate}}

%The following sets the labeling for inline enumerations
\setlist*[enumerate,1]{label=\it{\arabic*)}}

%Shortand sectioning command
\newcommand{\required}[1]{\section*{#1}}

%Change name of section for references
\renewcommand{\refname}{References Cited}

%Redefine \maketitle command
\makeatletter
\renewcommand{\maketitle}{\begin{center}\Large\textbf\@title
  \end{center}
  % Add author only if not empty (in the sense of producing output)
\setbox0=\hbox{\@author\unskip}\ifdim\wd0=0pt
\else
\begin{center}
  \@author
\end{center}
\fi%
}
\makeatother


==> preamble/proposalsSplitting.tex <==
%Package to get PDF page numbers
\usepackage{pageslts}
\pagenumbering{arabic}

%Macro to include file while writing to log file the splitting markers
\newcommand{\includeforsplit}[1]{%
  \typeout{Split marker [#1] [start] [\theCurrentPage]}%
  \setcounter{page}{1}%
  \setcounter{figure}{0}%
  \setcounter{table}{0}%
  \include{#1}%
  \clearpage
  \typeout{Split marker [#1] [end] [\theCurrentPage]}}


==> preamble/proposalsTaskSections.tex <==
%The following reformat the sections so that their labels read "Task x.y" instead of "x.y".
%Use the starred version of the command if you do not want this for
%some of the sections
\titleformat{\section}{\normalfont\large\bfseries}{Task \thesection:}{0.5ex}{}
\titleformat{\subsection}{\normalfont\bfseries}{Task \thesubsection:}{0.5ex}{}

